On Minimal Corrections in ASP

As a programming paradigm, answer set programming (ASP) brings about the usual issue of the human error. Hence, it is desirable to provide automated techniques that could help the programmer to find the error. This paper addresses the question of computing a subset-minimal correction of a contradictory ASP program. A contradictory ASP program is often undesirable and we wish to provide an automated way of fixing it. We consider a minimal correction set of a contradictory program to be an irreducible set of rules whose removal makes the program consistent. In contrast to propositional logic, corrections of ASP programs behave non-monotonically. Nevertheless, we show that a variety of algorithms for correction set computation in propositional logic can be ported to ASP. An experimental evaluation was carried showing that having a portfolio of such algorithms is indeed of benefit.

==> alg_x.tex <==
% File:  alg.tex
% Author: mikolas
% Created on: Wed, Feb 26, 2014 6:44:59 PM
% Copyright (C) 2014, Mikolas Janota
\begin{algorithm}[t]
  $P'\gets \maxim(\cR)$
}
\caption{Computing a Cardinality Maximal Model of $\cR$ for a program~$P$}\label{algorithm}
\end{algorithm}

